DarkQuest: A dark sector upgrade to SpinQuest at the 120 GeV Fermilab Main Injector

Expanding the mass range and techniques by which we search for dark matter is an important part of the worldwide particle physics program. Accelerator-based searches for dark matter and dark sector particles are a uniquely compelling part of this program as a way to both create and detect dark matter in the laboratory and explore the dark sector by searching for mediators and excited dark matter particles. This paper focuses on developing the DarkQuest experimental concept and gives an outlook on related enhancements collectively referred to as LongQuest. DarkQuest is a proton fixed-target experiment with leading sensitivity to an array of visible dark sector signatures in the MeV-GeV mass range. Because it builds off of existing accelerator and detector infrastructure, it offers a powerful but modest-cost experimental initiative that can be realized on a short timescale.

==> sections/todo.tex <==
\section*{List of action items}

\begin{itemize}
    \item More details on killing fake rates
    \item study of prompt dimuon at end of FMAG
\end{itemize}

% \begin{itemize}
%     \item \textbf{Nhan}: email E1039, start soliciting people who want to sign this white paper'
%     \item \textbf{Ming}: Ask Yu Dai if there will be a LongQuest ssection
%     \item \textbf{Stefania, Brian}, Section 2: add sterile neutrinos discussion
% \end{itemize}

% Beyond Mar 15: 
% \begin{itemize}
%     \item create big background sample (min Bias)
%     \item create neutral kaon background sample 
%     \item assess impact of additional tracking layer
% \end{itemize}


% Big questions to sort out with studies:
% \begin{itemize}
%     \item \textbf{Do we need another tracking layer before KMAG?} How much do DP1 and DP2 improve the tracking resolution 
% \end{itemize}

% \noindent Physics section
% \begin{itemize}
%     \item Need to re-organize physics benchmarks to be aligned with the RF6 "big ideas"
%     \item Explanation of assumptions that go into physics reach (trigger, reconstruction assumptions)
% \end{itemize}

% \noindent{Timeline}
% \begin{itemize}
%     \item First draft plots for Section~2,3,4 by Feb 4th
% \end{itemize}


